High-Quality Self-Supervised Deep Image Denoising

We describe a novel method for training high-quality image denoising models based on unorganized collections of corrupted images. The training does not need access to clean reference images, or explicit pairs of corrupted images, and can thus be applied in situations where such data is unacceptably expensive or impossible to acquire. We build on a recent technique that removes the need for reference data by employing networks with a "blind spot" in the receptive field, and significantly improve two key aspects: image quality and training efficiency. Our result quality is on par with state-of-the-art neural network denoisers in the case of i.i.d. additive Gaussian noise, and not far behind with Poisson and impulse noise. We also successfully handle cases where parameters of the noise model are variable and/or unknown in both training and evaluation data.

==> figures/gcrops/0-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc Kodak}-6}\hfill\makebox[\h]{20.41\,dB}\hfill\makebox[\h]{31.17\,dB}\hfill\makebox[\h]{31.17\,dB}\hfill\makebox[\h]{30.06\,dB}\hfill\makebox[\h]{29.04\,dB}\hfill\makebox[\h]{30.59\,dB}\vspace*{1mm}\\


==> figures/gcrops/10-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc BSD300}-18}\hfill\makebox[\h]{20.30\,dB}\hfill\makebox[\h]{31.98\,dB}\hfill\makebox[\h]{31.93\,dB}\hfill\makebox[\h]{30.77\,dB}\hfill\makebox[\h]{29.43\,dB}\hfill\makebox[\h]{31.30\,dB}\vspace*{1mm}\\


==> figures/gcrops/13-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc BSD300}-22}\hfill\makebox[\h]{20.58\,dB}\hfill\makebox[\h]{28.63\,dB}\hfill\makebox[\h]{28.57\,dB}\hfill\makebox[\h]{26.95\,dB}\hfill\makebox[\h]{25.07\,dB}\hfill\makebox[\h]{28.00\,dB}\vspace*{1mm}\\


==> figures/gcrops/16-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc BSD300}-28}\hfill\makebox[\h]{20.24\,dB}\hfill\makebox[\h]{26.78\,dB}\hfill\makebox[\h]{26.78\,dB}\hfill\makebox[\h]{24.16\,dB}\hfill\makebox[\h]{21.52\,dB}\hfill\makebox[\h]{26.37\,dB}\vspace*{1mm}\\


==> figures/gcrops/2-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc Kodak}-14}\hfill\makebox[\h]{20.42\,dB}\hfill\makebox[\h]{30.88\,dB}\hfill\makebox[\h]{30.80\,dB}\hfill\makebox[\h]{29.89\,dB}\hfill\makebox[\h]{28.98\,dB}\hfill\makebox[\h]{30.01\,dB}\vspace*{1mm}\\


==> figures/gcrops/20-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc BSD300}-80}\hfill\makebox[\h]{20.20\,dB}\hfill\makebox[\h]{32.75\,dB}\hfill\makebox[\h]{32.64\,dB}\hfill\makebox[\h]{31.81\,dB}\hfill\makebox[\h]{31.05\,dB}\hfill\makebox[\h]{32.03\,dB}\vspace*{1mm}\\


==> figures/gcrops/23-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc Set14}-2}\hfill\makebox[\h]{20.36\,dB}\hfill\makebox[\h]{31.60\,dB}\hfill\makebox[\h]{31.59\,dB}\hfill\makebox[\h]{31.30\,dB}\hfill\makebox[\h]{30.69\,dB}\hfill\makebox[\h]{32.06\,dB}\vspace*{1mm}\\


==> figures/gcrops/24-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc Set14}-5}\hfill\makebox[\h]{20.51\,dB}\hfill\makebox[\h]{29.44\,dB}\hfill\makebox[\h]{29.40\,dB}\hfill\makebox[\h]{28.34\,dB}\hfill\makebox[\h]{26.92\,dB}\hfill\makebox[\h]{28.09\,dB}\vspace*{1mm}\\


==> figures/gcrops/5-psnr.tex <==
% clean & noisy & n2c & unknown & diag_unknown & mean_only & bm3d & 
\scriptsize\makebox[\hh]{{\sc Kodak}-4}\hfill\makebox[\h]{20.35\,dB}\hfill\makebox[\h]{33.14\,dB}\hfill\makebox[\h]{33.09\,dB}\hfill\makebox[\h]{32.47\,dB}\hfill\makebox[\h]{31.86\,dB}\hfill\makebox[\h]{32.66\,dB}\vspace*{1mm}\\


==> figures/icrops/15-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-26}\hfill\makebox[\h]{12.08\,dB}\hfill\makebox[\h]{29.39\,dB}\hfill\makebox[\h]{28.88\,dB}\hfill\makebox[\h]{26.45\,dB}\vspace*{1mm}\\


==> figures/icrops/17-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-51}\hfill\makebox[\h]{10.96\,dB}\hfill\makebox[\h]{31.36\,dB}\hfill\makebox[\h]{30.74\,dB}\hfill\makebox[\h]{28.49\,dB}\vspace*{1mm}\\


==> figures/icrops/18-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-56}\hfill\makebox[\h]{11.07\,dB}\hfill\makebox[\h]{33.03\,dB}\hfill\makebox[\h]{32.64\,dB}\hfill\makebox[\h]{30.71\,dB}\vspace*{1mm}\\


==> figures/icrops/21-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-95}\hfill\makebox[\h]{10.31\,dB}\hfill\makebox[\h]{32.41\,dB}\hfill\makebox[\h]{31.92\,dB}\hfill\makebox[\h]{29.61\,dB}\vspace*{1mm}\\


==> figures/icrops/22-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc Set14}-1}\hfill\makebox[\h]{11.19\,dB}\hfill\makebox[\h]{23.96\,dB}\hfill\makebox[\h]{23.98\,dB}\hfill\makebox[\h]{21.81\,dB}\vspace*{1mm}\\


==> figures/icrops/25-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc Kodak}-20}\hfill\makebox[\h]{9.30\,dB}\hfill\makebox[\h]{34.90\,dB}\hfill\makebox[\h]{34.55\,dB}\hfill\makebox[\h]{32.13\,dB}\vspace*{1mm}\\


==> figures/icrops/26-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc Kodak}-19}\hfill\makebox[\h]{12.09\,dB}\hfill\makebox[\h]{33.62\,dB}\hfill\makebox[\h]{33.35\,dB}\hfill\makebox[\h]{31.08\,dB}\vspace*{1mm}\\


==> figures/icrops/3-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc Kodak}-15}\hfill\makebox[\h]{10.11\,dB}\hfill\makebox[\h]{35.13\,dB}\hfill\makebox[\h]{34.76\,dB}\hfill\makebox[\h]{32.84\,dB}\vspace*{1mm}\\


==> figures/icrops/7-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-4}\hfill\makebox[\h]{11.13\,dB}\hfill\makebox[\h]{34.41\,dB}\hfill\makebox[\h]{33.72\,dB}\hfill\makebox[\h]{31.86\,dB}\vspace*{1mm}\\


==> figures/pcrops/1-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc Kodak}-8}\hfill\makebox[\h]{18.63\,dB}\hfill\makebox[\h]{29.12\,dB}\hfill\makebox[\h]{29.11\,dB}\hfill\makebox[\h]{27.25\,dB}\vspace*{1mm}\\


==> figures/pcrops/11-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-19}\hfill\makebox[\h]{18.74\,dB}\hfill\makebox[\h]{29.49\,dB}\hfill\makebox[\h]{29.37\,dB}\hfill\makebox[\h]{27.46\,dB}\vspace*{1mm}\\


==> figures/pcrops/12-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-21}\hfill\makebox[\h]{19.33\,dB}\hfill\makebox[\h]{31.97\,dB}\hfill\makebox[\h]{31.81\,dB}\hfill\makebox[\h]{30.24\,dB}\vspace*{1mm}\\


==> figures/pcrops/14-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-25}\hfill\makebox[\h]{19.23\,dB}\hfill\makebox[\h]{26.75\,dB}\hfill\makebox[\h]{26.65\,dB}\hfill\makebox[\h]{23.31\,dB}\vspace*{1mm}\\


==> figures/pcrops/19-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-60}\hfill\makebox[\h]{18.10\,dB}\hfill\makebox[\h]{29.62\,dB}\hfill\makebox[\h]{29.61\,dB}\hfill\makebox[\h]{27.43\,dB}\vspace*{1mm}\\


==> figures/pcrops/2-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc Kodak}-14}\hfill\makebox[\h]{19.48\,dB}\hfill\makebox[\h]{30.33\,dB}\hfill\makebox[\h]{30.24\,dB}\hfill\makebox[\h]{28.64\,dB}\vspace*{1mm}\\


==> figures/pcrops/4-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc Kodak}-23}\hfill\makebox[\h]{19.13\,dB}\hfill\makebox[\h]{34.83\,dB}\hfill\makebox[\h]{34.63\,dB}\hfill\makebox[\h]{33.98\,dB}\vspace*{1mm}\\


==> figures/pcrops/6-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-3}\hfill\makebox[\h]{21.87\,dB}\hfill\makebox[\h]{28.57\,dB}\hfill\makebox[\h]{28.43\,dB}\hfill\makebox[\h]{23.91\,dB}\vspace*{1mm}\\


==> figures/pcrops/8-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-7}\hfill\makebox[\h]{17.81\,dB}\hfill\makebox[\h]{29.39\,dB}\hfill\makebox[\h]{29.26\,dB}\hfill\makebox[\h]{27.01\,dB}\vspace*{1mm}\\


==> figures/pcrops/9-psnr.tex <==
% clean & noisy & n2c & unknown & mean_only & 
\scriptsize\makebox[\hh]{{\sc BSD300}-11}\hfill\makebox[\h]{19.91\,dB}\hfill\makebox[\h]{31.72\,dB}\hfill\makebox[\h]{31.63\,dB}\hfill\makebox[\h]{30.01\,dB}\vspace*{1mm}\\

